Amodal Completion and Size Constancy in Natural Scenes

We consider the problem of enriching current object detection systems with veridical object sizes and relative depth estimates from a single image. There are several technical challenges to this, such as occlusions, lack of calibration data and the scale ambiguity between object size and distance. These have not been addressed in full generality in previous work. Here we propose to tackle these issues by building upon advances in object recognition and using recently created large-scale datasets. We first introduce the task of amodal bounding box completion, which aims to infer the the full extent of the object instances in the image. We then propose a probabilistic framework for learning category-specific object size distributions from available annotations and leverage these in conjunction with amodal completion to infer veridical sizes in novel images. Finally, we introduce a focal length prediction approach that exploits scene recognition to overcome inherent scaling ambiguities and we demonstrate qualitative results on challenging real-world scenes.

==> applications.tex <==
\section{Applications}
Cool figures: 
1) Make scenes 3D
2) Run it on new datasets e.g. COCO


==> related.tex <==
\section{Related Work}


Hoiem et al \cite{hoiem2008putting} studied the interaction between object detection and scene layout estimation and showed that reasoning over object sizes within their 3D environment, as opposed to within the image, had a positive impact on detection performance. 

The work Lalonde et al \cite{lalonde2007photo} is close to ours. It estimates average real world sizes of many object categories in the 3D world, from annotated LabelMe data.

This was still in the HOG age  \cite{dalal2005histograms} -- here we leverage the more powerful feature extraction technology we have now to be able to widthstand occlusions and recover metric information.

Building a database of 3d scenes from user annotations \cite{russell2009building}. This is a heavy duty system with quite a broad model, that classifies pairwise relationships into support, attachment, occlusion, etc. On the bright side it assumes every pixel is annotated as belonging in a region. It also does not perform completion and it's not clear  exactly how they recover depth of occluded objects, probably using familiarity, etc.. ?
 
 Other references:
-  Are Cars Just 3D Boxes? – Jointly Estimating the 3D Shape of Multiple Objects. Schindler
-  Towards Scene Understanding with Detailed 3D Object Representations. Schindler
------------------------------------------------------

Psychology:
Do Artists See Their Retinas? Cavanagh

Amodal completion:
Amodal volume completion: 3D visual completion. Fisher


Organization in vision: Essays on Gestalt perception. Kanizsa 1979

%
